Cartolabe: A Web-Based Scalable Visualization of Large Document Collections

We describe CARTOLABE, a web-based multi-scale system for visualizing and exploring large textual corpora based on topics, introducing a novel mechanism for the progressive visualization of filtering queries. Initially designed to represent and navigate through scientific publications in different disciplines, CARTOLABE has evolved to become a generic framework and accommodate various corpora, ranging from Wikipedia (4.5M entries) to the French National Debate (4.3M entries). CARTOLABE is made of two modules: the first relies on Natural Language Processing methods, converting a corpus and its entities (documents, authors, concepts) into high-dimensional vectors, computing their projection on the 2D plane, and extracting meaningful labels for regions of the plane. The second module is a web-based visualization, displaying tiles computed from the multidimensional projection of the corpus using the U MAP projection method. This visualization module aims at enabling users with no expertise in visualization and data analysis to get an overview of their corpus, and to interact with it: exploring, querying, filtering, panning and zooming on regions of semantic interest. Three use cases are discussed to illustrate CARTOLABE's versatility and ability to bring large scale textual corpus visualization and exploration to a wide audience.

==> 0-discuter.tex <==
web ou Web: partout un W ou partout un w.
Pas du tout d'accord pour mettre Sebag comme référence. Le star système ?



===========
Use case, line 37: combien ?
Je ne comprends pas s'il est disponible, si l'exe est disponible, si le code est disponible...
Conclusion, l. 6.

========
comprend pas comment faire marcher les \label et \ref

Rajouter une ref sur stressed, les dechirures etc.

qu'est-ce que le viewport ?

periode des articles publi'es ds Hal: [2008-now] ? file 03-B line 49.

Pas Michele Sebag. Leslie Lamport; ou qq'un connu pour le champ du journal.

==> 00-notes.tex <==
A Intro.

B (en section 2 ou `a la fin: state of the art: 
qui les compétiteurs; quelles données; quelles techniques (graphe, full text; 
Qui est out of scope. ex, Politoscope Tweets)

C Overview, Architecture / Pipeline; profils d'usage; 
* cherche un reviewer ou un partenaire industriel
* tete d'organisme, qu'est-ce qu'on sait faire;
* directeur stratégique, ou on va, ce qui est chaud. 
Les fonctionnalités s'en déduisent (normalement).

D Exploratory Data Analysis/Machine Learning
E Visualisation
(on peut swapper)

F Use cases: Strengths and Weaknesses
qq mots sur les domaines; forces et limites de l'approche 

[Validation]

Discussion; Limites et Perspectives


==> 04-visu.tex <==
\section{Visualization}\label{sec:visu}

\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{filter}
  \caption{Cartolabe can generate filtered density maps based on a user query. RoaringBitmaps are used to store indices of points matching possible filter values. Upon query, the filtered point indices are lookedup and their position is used with the Datashader library to create a tiled overlay showing the density map for the filtered points.}
  \label{fig:filter}
\end{figure*}


The data managed by Cartolabe is a set of points, each point having a label, a type, 2D coordinates, a score to represent its importance and a list of nearest neighbors for each point type. The goal of the Cartolabe application is to provide a meaningful, interactive visualization of this generic dataset. This simple data structure makes it easy for the Cartolabe application to become domain independent and thus apply to all kinds of data, as long as they can be represented as a list of entities with coordinates.

As mentioned previously, if the distance that separates the points in the dataset can be made to represent content, then the shape of the visualization becomes significant. This is done by using dimension reduction techniques for visualization such as t-SNE \cite{tsne} or UMAP \cite{2018arXivUMAP}. This way, points that are close together in the high dimensional space will be close together on the map (though these techniques are never perfect and have some artifacts). This means that Cartolabe can provide some interesting overview of the dataset by showing significant regions of content. This type of visualization though is most often meaningful for high level representations which show the totality of the dataset. Being able to display as many points as possible is therefore important for this visualization.

Cartolabe manages this by creating density map images from the dataset to represent the distribution of points. A library like Datashader \cite{datashader} is specifically designed for such usage. The Datashader library can easily plot millions of points into a single image. But the drawback from such images is that they do not allow for easy exploration of the dataset. In order to be able to zoom into a region and see only the points in this area, a new image needs to be generated from the restricted data. To provide interaction, Cartolabe uses a Javascript map tiling library \cite{d3} to display the static images generated by Datashader as an interactive map. Static images of the dataset are generated offline with increasing width and height for each successive zoom level \(z \geq 0\). These images are then cut up into \(2^z * 2^z\) tiles of the same size (\(256 * 256\) pixels). Cartolabe is thus able to display a single image tile at zoom level 0, \(2 * 2\) tiles at zoom level 1, \(4 * 4\) tiles at zoom level 2 … Figure \ref{fig:tiles} shows such a tile pyramid.

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{tiles}
  \caption{Tile pyramids, commonly used for zoomable map applications, can also be adapted to display high resolution images. Images of increasing resolution are cut up into an increasing number of tiles to form a tile pyramid. Zooming and scrolling functions are thus a matter of displaying the tiles corresponding to the zoom level and position of the viewport.}
  \label{fig:tiles}
\end{figure}

This interactivity means that the user is able to dive into the data and look for a specific region or point. But of course, it is then necessary to provide contextual information for the user to be able to identify the region or point that is currently displayed on the screen. This is done by displaying labels on top of the tiled density maps to identify such regions and points. Because of the high number of points which can sometimes be visible on the screen, it is not possible to display the labels for all of them at the same time. This is why scores are associated with each point to represent its supposed interest for the user. For the HAL dataset, the score of an article can be set to its citation count. In a certain viewport, only a limited number of labels are displayed with points having the highest score being displayed in priority. The same goes for the cluster labels which are essential to identify meaningful areas. Different levels of importance for the clusters help select which labels to display per zoom level. Cartolabe relies on an Elasticsearch database to be able to search and filter points by score and position. The scalability and efficiency of Elasticsearch makes it easy to request a limited number of important points to display in a specific viewport.


Managing contextual filters as described in Figure \ref{fig:cern} requires a bit more work. As mentioned before, this is an essential part of the visualization engine for Cartolabe as it lets the user filter the density maps to only display points which match a certain criterion. In the example for Figure \ref{fig:cern}, we filter the map based on a laboratory: only articles and authors associated with the CERN lab are displayed. The HAL dataset contains more than 10000 labs which the user could potentially filter on. Other filter values can also be used, for example the HAL dataset can also be filtered based on publication year for the articles. It is also possible to combine filter values and for example visualize the points associated with the CERN or INRIA labs and published in 2018. For obvious reasons, pre-generating the density maps for all possible filter value combinations is not feasible. Density maps thus need to be generated online as the user requests them. In order to achieve this, Cartolabe relies on RoaringBitmaps \cite{Lemire2018} to create and store compressed indices of the point ids associated with each possible filter value. RoaringBitmaps offer a memory and time efficient solution for this, allowing bitwise operations to be performed on the sets in near-constant time regardless of size. For Cartolabe, this means that we are able to keep track of the ids of all articles associated with the CERN laboratory in one bitmap, as well as the ids of all articles published in 2018 in another bitmap, and easily combine them to get the ids of CERN articles published in 2018.

Once we know the ids of points which match the filter values, it is only a matter of creating the density map images to display in the viewport. Because the Datashader library is quite efficient at generating density images, this can be done in reasonable time (\(\leq 500ms\)) by first filtering out the points outside the viewport. We again use RoaringBitmaps to keep indices of all the points located in each map tile. We are thus able to efficiently filter the previous set of points to only keep the ones that are within a certain range of coordinates. We use this filtered set of points with Datashader to create a tiled portion of the density map matching the user’s criteria and we display it on top of the shaded overall map. This process, summarized in Figure \ref{fig:filter}, is repeated each time the user zooms in or scrolls the map, with limited caching to improve performance.





==> 05-pipeline.tex <==
\section{Cartolabe-data: Text Processing Pipeline}\label{sec:pipeline}

In this section we describe the process of transforming a text corpus into a collection of points usable by the Cartolabe visualization engine. This process is summarized in Figure \ref{fig:pipeline} applied to the HAL dataset. 

The key aspect of the data processing pipeline are:
\begin{itemize}
\item An homogeneous representation of all the entities (articles, authors, words, ...) in three different spaces (see section \ref{sec:spaces})
\item Landmarks (section \ref{sec:clustering}) and entity scoring (section \ref{sec:scoring}) to ease the exploration of the map 
\item A flexible pipeline using state-of-the-art modules to be able to scale up to millions of entities (e.g., Scikit-Learn\cite{scikit-learn} for text processing and dimensionality reduction, UMAP for multidimensional scaling and approximate KNN\cite{ann} neighbors computing) (see sections \ref{sec:text} to section \ref{sec:export})
\item The homogeneous representation and the flexibility of the pipeline is designed to be easily changed, for other applications or to test other algorithms at each step (see how several use cases differ from the HAL application presented here in section \ref{sec:usecases}).
\end{itemize}


\subsection{Entities and representation spaces}
\label{sec:spaces}
The input of the pipeline will be a set of $T$ documents (articles), with meta-data about other entities: authors, labs, ... This will define the set 
%E={Earticles, Ewords, .. , Eauthors} 
of entities which will be processed almost homogeneously and represented on the final map. On the HAL dataset we have 4 main type of entities: $articles$, $words$ (each $word$ entity is a ngram composed of one or several words), $authors$ and $laboratories$. 4 level of $clusters$ are also defined as entities (high, medium, low and very low level clusters). However, these entities do not need representation in the natural and latent space (see bellow). Such representation could still be inferred if needed (for example to compute the nearest cluster for each entity). 

All entities (except clusters) have three representations:
\begin{itemize}
    \item $natural$ space (sparse, dimension: $T$=number of articles). The first step of of the pipeline builds a representation of the text documents in the corpus as a matrix of token counts. This builds the $natural$ space representation composed of high-dimension sparse matrices. Each entity has a representation in this natural (article) space: identity for the articles, TF-IDF word extractions for the words, authorship for the authors, .... 
    \item $latent$ space (dense, dimension $d\approx$200-500). Dimensionality reduction (LSA) or Topic modeling algorithms (LDA) are used to reduce this natural space to a $latent$ space. This latent space is composed of dense matrices with a limited number (200-500) of components. This space is used to compute similarities between entities (compute the neighbors).
    \item $2D$ space (dense, dimension:2). Multidimensional scaling algorithms are used to compute the projection from the latent space into 2D space. The 2D space is used to display entities on the map, but also to compute the clusters used to display Landmark names on the map.
\end{itemize}

%One of the key aspect of the Cartolabe-data pipeline is the distinction of these three representation spaces: the sparse $natural$ space is used almost only to construct the latent space. The $latent$ space is used as the main working space, to compute similarities between entities (authors, articles). The $2D$ space is the final visualisation space.

%In this section we describe the process of transforming a text corpus into a collection of points usable by the Cartolabe visualization engine. This process is summarized in Figure \ref{fig:pipeline}. The first step of this process builds a representation of the text documents in the corpus as a matrix of token counts. This builds the natural space representation composed of high-dimension sparse matrices. We then use topic modeling algorithms to reduce this natural space to a latent space. This latent space is composed of dense matrices with a limited number (200-500) of components. Once this is done, we can then run clustering and nearest neighbor algorithms on our documents. Finally, we use dimensionality reduction algorithms to assign 2D coordinates to each document. We manage related entities to each document (authors, labs, etc.) by simply mapping the coordinates of each entity to the coordinates of its related documents.

\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figures/Cartolabe-shemas.png}
  \caption{Cartolabe data processing pipeline, applied to the HAL dataset.}
  \label{fig:pipeline}
\end{figure*}

\subsection{Raw text processing and entity mapping}
\label{sec:text}

The first step of the pipeline is to represent all entities as a composition of articles (the (sparse) natural space of dimension $T$). The representation of the article entities in this space will trivially be the Identity matrix $I_T$.


\subsection{Dimensionality reduction}


LDA can also be used for the dimensionality reduction. The result of the analysis is topic representation of both words and articles entities. In this case, several possibilities can be used to project the other entities, for example to use the topic representation of the articles (dimension (T,d)) as the projection matrix. 

For the current use cases, LSA dimensionality reduction was selected after qualitative evaluation of the final maps.   



\subsection{Scoring}
\label{sec:scoring}
The score of each entity is used to select the apparition order on the map:
\begin{itemize}
    \item The score of the authors and labs is the number of articles they wrote.
    \item The score of the words is the number of articles where they appear.
    \item The score of the articles is \rev{the average number of views in HAL per year}. \del{always 1 (no metadata is publicly available in HAL concerning the citations or the number of views of each article).}
\end{itemize}


\subsection{2D projection}

To be displayed on the map, latent space coordinate matrix of all entities have to be projected into 2D space.

Multidimensional scaling 2D reduction techniques such as t-SNE  and UMAP~\cite{2018arXivUMAP} can be used to visually represent high dimension data in a 2- or 3-dimension space by preserving close neighbors (and neglecting higher distance values). 
We use the UMAP algorithm algorithm, which can be trained on a subset of points and applied on the full set while keeping its good projection properties. For our larger datasets (more than 1-2 million points, like the Grand D\'ebat use case, see section \ref{sec:granddebat}), we train the model on a subset of the data and then apply the model for the remaining data points.

\subsection{Clustering}
\label{sec:clustering}

To understand the map, it is important to provide Landmarks/names that will describe the group of points nearby. 
To achieve this, clusters of articles are computed and a name is associated with each cluster. To provide landmarks at several zoom levels, several clustering are computing with increasing number of clusters (4 levels with 8 to 512 clusters for HAL).

Clusters are computed using K-means algorithm on all articles in the 2D space. We use 2D space rather than latent space to compute the clusters, because latent space clusters are often projected in several regions of the 2D map, which is much less usefull to profide landmarks and clear identification. 2D clusters are well separated and provide useful landmarks, even if they can miss some groups that would have been identified if the clusters were computed in the latent space.

Each level clustering and naming is a 4 step process, :
\begin{itemize}
    \item Compute the k clusters $C_{1..k}$ using K-means on the articles 2D space matrix.
    \item Apply the k-means trained on the articles on the $word$ 2D space matrix to associate each word with a cluster.  
    \item For each cluster, select $word$ entity associated with the cluster $v$ that is most present in the cluster but not outside the cluster (proportion of articles in the cluster with the term-proportion of articles in the corpus with the term). If there is no $word$ in the cluster, select from the $word$ entities not associated with the cluster that is not already used as a label.
    \item For each cluster, if less than half the articles use the selected $word$, select an other $word$ using the same methodology on the remaining articles.
\end{itemize}

For each cluster, we get a 2D coordinate (cluster centroid) and a name with one or two $words$ (ngrams). With several level of clusters, this provides landmarks for different zoom levels.

%Clustering is a common part of any machine learning task and it is essential to Cartolabe. We rely on a standard K-means algorithm to detect clusters. But rather than the clustering algorithm used, Cartolabe is more concerned with the method used to label the clusters resulting from it. Cluster labels are essential to make the map generated by this pipeline understandable. Without visible landmarks, the density maps displayed by the visualization engine resemble a night sky and as the user zooms in, it is difficult to know which part of the data is being explored. Cluster labels are used to identify semantic areas in the map. The method adopted by Cartolabe is to select one or two terms with the highest TF/IDF score which were classified in each cluster. This ensures that the most semantically significant terms are used as labels for a cluster. In order to avoid duplicate labels, we filter out identical terms from appearing twice in cluster labels.

%In order to provide clustering that is adapted to each zoom level of the map when displayed in Cartolabe, we run the clustering task several times with an increasing number of clusters. This ensures that more generic classes will be displayed at lower zoom levels, while zooming in will allow to display more and more specific classes.

\subsection{Export}
\label{sec:export}
A file is generated to be used by the cartolabe-vis server. For each entity, it contains:
\begin{itemize}
    \item Its label, score, position (2D), type (article/author/\ldots)
    \item Its neighbors
    \item To generate the density maps, the related entities (e.g., for HAL, for each lab, the ids of all its articles and authors). 
    \item Some metadata to be displayed (e.g., HAL link for the articles).
\end{itemize}
Depending on the size, we can use JSON or the more compact Feather format.
